Tracing where IoT data are collected and aggregated

The Internet of Things (IoT) offers the infrastructure of the information society. It hosts smart objects that automatically collect and exchange data of various kinds, directly gathered from sensors or generated by aggregations. Suitable coordination primitives and analysis mechanisms are in order to design and reason about IoT systems, and to intercept the implied technological shifts. We address these issues from a foundational point of view. To study them, we define IoT-LySa, a process calculus endowed with a static analysis that tracks the provenance and the manipulation of IoT data, and how they flow in the system. The results of the analysis can be used by a designer to check the behaviour of smart objects, in particular to verify non-functional properties, among which security.

==> sections/proof-vecchia.tex <==
% !TEX root = ../main_coord2016.tex
%
In this appendix, we restate the theorems presented earlier
in the paper, include the needed lemmata and give the proofs of their correctness. 

%The proofs benefit from an instrumented denotational semantics for expressions, the values of which are pairs $\langle v, \hat{v}\rangle$.
%Consequently, the store ($\Sigma^i_\ell$ with a $\bot$ value to record that a sensor or a variable is not initialized) and its updates are accordingly extended
%(the semantics used in \tablename~\ref{opsem} is $\dsem{v}^i _{\downarrow_1}$, the projection on the first component of the instrumented one).
%The instrumented local store then becomes: 
%$
%\Sigma^{i}_{\ell} : \mathcal{X} \cup \mathcal{I} _\ell\ \rightarrow \mathcal{V} \times \hat{\mathcal V}.
%$ 
%%
%The formal definition of the instrumented denotational semantics follows.
%%%
%\[
%\begin{array}{lll}
%\dsem{v}^i_{\Sigma^{i}_{\ell}} & = & (v, v^\ell)
%\\
%\dsem{i}^i_{\Sigma^{i}_{\ell}} & = & \Sigma_{\ell}^i(i)
%\\
%\dsem{x}^i_{\Sigma^{i}_{\ell}} & = & \Sigma_{\ell}^i(x)
%\\
%\dsem{f(E_1,\cdots, E_k)}^i_{\Sigma^{i}_{\ell}} & = & 
%(f(\dsem{E_1}^i_{\Sigma^{i}_{\ell} \downarrow_1},\cdots, \dsem{E_k}^i_{\Sigma^{i}_{\ell} \downarrow_1}),
%\lfloor f^{\ell}(\dsem{E_1}^i_{\Sigma^{i}_{\ell} \downarrow_2},\cdots,\dsem{E_k}^i_{\Sigma^{i}_{\ell} \downarrow_2})\rfloor_{d})
%\end{array}
%\]
%%%%%%%%%% DEF + STRETTA %%%%%%%%%%%%
%%\[
%%\begin{array}{l}
%%\dsem{v}^i_{\Sigma^{i}_{\ell}}  =  (v, v^\ell)
%%\qquad\qquad\qquad
%%\dsem{i}^i_{\Sigma^{i}_{\ell}}  =  \Sigma_{\ell}^i(i)
%%\qquad\qquad\qquad
%%\dsem{x}^i_{\Sigma^{i}_{\ell}}  =  \Sigma_{\ell}^i(x)
%%\\
%%\dsem{f(E_1,\cdots, E_k)}^i_{\Sigma^{i}_{\ell}}  =  
%%(f(\dsem{E_1}^i_{\Sigma^{i}_{\ell} \downarrow_1},\cdots, \dsem{E_k}^i_{\Sigma^{i}_{\ell} \downarrow_1}),
%% f^{\ell}(\dsem{E_1}^i_{\Sigma^{i}_{\ell} \downarrow_2},\cdots,\dsem{E_k}^i_{\Sigma^{i}_{\ell} \downarrow_2}))
%%\end{array}
%%\]
%%
%
%\noindent
%Since the CFA only considers the second component of the extended store, we need to define when the concrete and the abstract stores agree.
%
%\begin{definition}
%Given a concrete store $\Sigma_\ell^i$ and an abstract store $ \hat{\Sigma_\ell}$, we say that
%they {\em agree}, in symbols
%$\Sigma_\ell^i \bowtie \hat{\Sigma_\ell}$ if and only if for all
%$w \in \mathcal{X} \cup \mathcal{I} _\ell$ either $\Sigma^i_\ell (w) = \bot$
%or there exists $\hat{G} \in \hat{\Sigma}_\ell(w)$ such that 
%$(\Sigma^i_\ell (w))_{\downarrow_2} \in  Lang(\hat{G})$.
%\end{definition}
%

\noindent Before proving the correctness of the analysis, we prove that it is invariant under the structural congruence and is preserved under node components reduction.

\begin{lemma}[Congruence]\label{lemma:congr}\ \\
\begin{itemize}
\item
If $B \equiv B'$ then
$\nPAFORM{\ell}{B}$ iff $\nPAFORM{\ell}{B'}$.
\item
If $N \equiv N'$ then
$\nNAFORM{N}$ iff $\nNAFORM{N'}$.
\end{itemize}
\end{lemma}
\begin{proof} 
It suffices to inspect the rules for $\equiv$, since
associativity and commutativity of $\wedge$
reflects the same properties of both $|$ and $\|$, and to recall that any triple is a valid
estimate for $\NIL$.  
\end{proof}

\begin{lemma}[Subject reduction for node components]\label{SRtheoremB}\ \\
If $\nPAFORM{\ell}{B}$ and $B \sfreccia B'$ and $\Sigma_\ell^i \bowtie \hat{\Sigma_\ell}$, for $\Sigma_\ell^i$ {\em ($in$ $B$)}
then $\nPAFORM{\ell}{B'}$ and $\Sigma{_\ell^i}' \bowtie \hat{\Sigma_\ell}$, for $\Sigma{_\ell^i}'$ {\em ($in$ $B'$)}.
\end{lemma}
\begin{proof} 
Our proof is by induction on the shape of the derivation of $B \sfreccia B'$ and by cases on the last rule used.
In all the cases below we will have that for $\Sigma^{i}$ and $B_1$ components of $B$, the following trivially hold (*) $\nPAFORM{\ell}{\Sigma^{i}}$, and (**) $\nPAFORM{\ell}{B_1}$.
So we will omit mentioning these judgements.
\\
%\begin{itemize}
%\item
- Case (Sense). We assume 
$\nPAFORM{\ell}{\Sigma^{i} \parallel probe(i).\, S \parallel B_1 }$ that has been proved because $\nPAFORM{\ell}{probe(i).\, S}$ holds.
%
This implies that $\nPAFORM{\ell}{S}$ holds, and thus
$\nPAFORM{\ell}{\Sigma^{i}\{(v,i^\ell)/{i}\} \parallel S \parallel B_1}$.
We are left to show that
$\Sigma{_{\ell}^i}' \bowtie \hat{\Sigma_{\ell}}$.
By hypothesis $\Sigma{_{\ell}^i}' (y)= \Sigma{_{\ell}^i}(y)$ for all $y \in {\mathcal X}_{\ell} \cup {\mathcal I}_{\ell}$ such that $y \neq i$, 
while $(\Sigma^i_{\ell} (i))_{\downarrow_2} = i^\ell \in Lang(\hat{G})$, for some $\hat{G} \in \hat{\Sigma}_{\ell}(i)$, which \mbox{trivially holds by (*).}\\
%\item
- Case (Asgm). We assume 
$\nPAFORM{\ell}{\Sigma^{i} \  \|\  x:=E.\,P \  \|\ B_1 }$
that has been proved because the following conditions hold:         
\begin{eqnarray}
&& \nEFORM{E}{\vartheta} \label{c1}
\\
&&\forall \hat{v}:\; \hat{v} \in \vartheta\ \Rightarrow
\hat{v} \in \hat{\Sigma}{_\ell}({x})\hspace*{4ex} \label{c2}\\
&& \nPAFORM{\ell}{P}\label{c3}
\end{eqnarray}
%
We have to prove that
$\nPAFORM{\ell}{\Sigma^{i}\{(v,\hat{v})/x\} \  \|\  P \  \|\ B_1 }$ that trivially holds because of (*), (\ref{c3}) and (**), respectively.
We have only to prove that
$\Sigma{_{\ell}^i}' \bowtie \hat{\Sigma_{\ell}}$, by knowing that (by hypothesis) $\Sigma{_{\ell}^i} \bowtie \hat{\Sigma_{\ell}}$, that implies
$\Sigma{_{\ell}^i}' (y)= \Sigma{_{\ell}^i}(y)$ for all $y \in {\mathcal X}_{\ell} \cup {\mathcal I}_{\ell}$ such that $y \neq x$.
Therefore $\Sigma{_{\ell}^i}' (y)= \Sigma{_{\ell}^i}(y)$ for all $y \in {\mathcal X}_{\ell} \cup {\mathcal I}_{\ell}$ such that $y \neq x$,
while $(\Sigma^i_{\ell} (x))_{\downarrow_2} \in  Lang(\hat{v} \in \hat{\Sigma}_{\ell}(x))$ because of (\ref{c2}).
\\
%\item
- Case (E-out). We assume 
$\nPAFORM{\ell}{\Sigma^{i}  \  \|\   \OUTM{E_1,\! \cdots \!,E_r}{L}. \, P \  \|\  B_1}$
         %
that has been proved because the following conditions hold:       
\begin{eqnarray*}
&& - \bigwedge_{i=1}^r\; \nEFORM{E_i}{\vartheta_i} \\
&& - \  \nPAFORM{\ell}{P}
\\
&& - \  \forall \hat{v}_1,\cdots,\hat{v}_r:\; \bigwedge_{i=1}^r\, \hat{v}_i \in \vartheta_i\ \Rightarrow
\forall \ell' \in L:
         (\ell,  \mess{\hat{v}_1,\cdots,\hat{v}_r}) \in  \kappa(\ell')
\end{eqnarray*}
%
Proving that
$
\nPAFORM{\ell}{\OUTM{v_1,\cdots,v_r}{L}. \, \NIL  \ \| \ \ P \ \| \ B_1}
$
is straightforward because of the three above conditions.
%Also, the condition on the stores trivially holds, since 
%the store in the node $\ell$ does not change.
\\
%\item
- The cases (ParB), (StructB) directly follow from the induction hypothesis; the case (CongrB) from Lemma \ref{lemma:congr}, and the remaining ones are straightforward.
%\end{itemize}
\end{proof}


\subjectreduction*
\begin{proof} 
Our proof is by induction on the shape of the derivation of $N \sfreccia N'$ and by cases on the last rule used.
In all the cases below we will have that (*) $\nPAFORM{\ell}{\Sigma^{i}}$, as well as that (**) $\nPAFORM{\ell}{B_1}$ and $B_2$, for $\Sigma^i, B_1, B_2$ components of $N$.
So we will omit mentioning these judgements.
\\
- Case (Multi-com). We assume
\[
\!\!\! \nNAFORM{\ell_1 \! : \!  [\OUTM{v_1,\! \cdots \!,v_r}{L}. \, \NIL \  \|\  B_1]\ | \
             \ell_2  \! : \! [\Sigma^{i}_2 \ \| \ (E_1,\! \cdots \!,E_j;x_{j+1},\! \cdots \!,,x_r).Q \ \| \ B_2]}
             \] 
that is implied by
$\nNAFORM{ \ell_1: [\OUTM{v_1,\cdots,v_r}{L}. \, \NIL \  \|\  B_1]}$ and by\\
             $\nNAFORM{\ell_2:[\Sigma^{i}_2 \ \| \ (E'_1,\cdots,E'_j;x_{j+1},\cdots,x_r).Q \ \| \ B_2]}$
that have been proved because the following conditions hold:      
 
\begin{eqnarray}
&& \bigwedge_{i=1}^r\; \nEFORMM{\ell_1}{v_i}{\vartheta_i} \label{c5}
\\   
&& \nPAFORM{\ell_1}{\NIL}\label{c7}
\\
&& 
\forall \hat{v}_1,\cdots,\hat{v}_r:\; \bigwedge_{i=1}^r\, \hat{v}_i \in \vartheta_i\ \Rightarrow
\forall \ell' \in L:
         (\ell_1,  \mess{\hat{v}_1,\cdots,\hat{v}_r}) \in  \kappa(\ell')  \hspace*{4ex} \label{c6}
\\
&& \bigwedge_{i=1}^{j}\;  \nEFORMM{\ell_2}{E_i}{\vartheta'_i} \label{c8}
\\[2ex]
 && Comp(\ell_1,\ell_2)\label{c4}
\\
%&&\forall (\ell', \mess{ \hat{v} _1,\cdots,\hat{v}_k}) \in \kappa(\ell_2) :\;
%	  \bigwedge_{i=1}^{j}\;  \hat{v}_i \in \vartheta'_i\  \Rightarrow  \label{c9}
%	  \\[-4ex]
& &  \bigwedge_{i=j+1}^r\;  \hat{v}_i \in \hat{\Sigma}{_{\ell_{2}}}({x_i}) \label{c10} \ \\
& &  \nPAFORM{\ell_2}{Q} \label{c11}
\end{eqnarray}
%
Note that since~\ref{c4} holds, also \ref{c10} and~\ref{c11} do.
Also, $\forall i\; \nEFORMM{\ell_1}{v_i}{\vartheta_i}$ implies $\hat{v}_i \in \vartheta_i$, 
where $\hat{v}_i = (\dsem{v_i}^i_{\Sigma^{i}_{\ell_{2}}})_{\downarrow_2}$, and that $\ell_2 \in L$ because $N \sfreccia N'$.
%
%The premise of (Multi-com) ensures that
%$\ell_2 \in L$, $Comp(\ell_1,\ell_2)$, and $\bigwedge_{i=1}^{j} {(v_i, \hat{v}_i)}= \dsem{E_i}_{\Sigma_2}$, and therefore 
%$\bigwedge_{i=1}^j\ \hat{v_i} \in \vartheta'_i$ follows.
We have to prove that
\[
\!\!\! \nNAFORM{\ell_1: [\OUTM{v_1,\cdots,v_r}{L \setminus \{\ell_2\}}. \NIL   \|  B_1]
              \ | \ \ell_2: [\Sigma^{i}_2\{v_{j+1}/x_{j+1},\cdots,v_r/x_r\}  \|  Q \|  B_2]}
\]              
that in turn amounts to prove that
%
\[
\begin{array}{l}
(a)\ \nPAFORM{\ell_1}{\OUTM{v_1,\cdots,v_r}{L \setminus \{\ell_2\}}. \,\NIL  \ \| \ B_1 } 
\\
(b)\  \nPAFORM{\ell_2}{ \Sigma^{i}_2\{(v_{j+1}, \hat{v}_{j+1})/x_{j+1},\cdots,(v_r, \hat{v}_r)/x_r\} \ \| \ Q\ \| \ B_2 }
\end{array}
\]    
%
We have that $(a)$ holds trivially because of (\ref{c5}),~(\ref{c7}) and~(\ref{c6}) (of course $L\setminus \{ \ell_2\} \subseteq L$), while
$(b)$ holds because of the remaining conditions.
We are left to prove that
$\Sigma{_{\ell_{2}}^i}' \bowtie \hat{\Sigma}_{\ell_{2}}$.
Now, we know that $\Sigma{_{\ell_{2}}^i}' (y)= \Sigma{_{\ell_{2}}^i}(y)$ for all $y \in {\mathcal X}_{\ell_{2}} \cup {\mathcal I}_{\ell_{2}}$ such that $y \neq x_i$.
The condition $(\Sigma^i_{\ell_2} (x_i))_{\downarrow_2} \in  Lang(\hat{v} \in \hat{\Sigma}_{\ell_2}(x_i))$ holds for all $x_i$  
because of (\ref{c10}).
\\
- The case (CongrN) follows from Lemma \ref{lemma:congr}.
\\
- The remaining cases directly follow from the induction hypothesis.
%\end{itemize}
\end{proof}

The following auxiliary lemma helps proving Corollary~\ref{cor:Theta}, and in its statement we let $B \xrightarrow{E_1, ...,E_n}_\ell B'$ denote a reduction in which all $E_i$ are evaluated at node $\ell$, omitting the environment.

\begin{lemma}\label{cor:ThetaB}\ \\
If $\nPAFORM{\ell}{B}$ and $B \xrightarrow{E_1, ...,E_n}_\ell  B'$ then $\forall k \in [0,n]$ 
there exists $\hat{G} \in \Theta(\ell)$ such that
$(\dsem{E_r}^i_{\Sigma^i_\ell})_{\downarrow_2} \in Lang(\hat{G})$.
\end{lemma}

\begin{proof}
By Lemma~\ref{SRtheoremB}, $\nPAFORM{\ell}{B'}$ holds. 
The proof proceeds by induction on the shape of the derivation of $B \sfreccia B'$ and by cases on the last rule used.
\\
- {Case} (Asgm).
If this rule is applied, then 
$B =  \Sigma^{i} \  \|\  x:=E.\,P \  \|\ B_1.
$
Since 
$
\nPAFORM{\ell}{B}
$
we have that, in particular, 
$\nPAFORM{\ell}{x : = E}.\,{P}$ and in turn that 
$ \nEFORM{E}{\vartheta}$.
By the rules in \tablename~\ref{analysisT}, we have 
the required  $\vartheta \subseteq \Theta(\ell)$.
\\
- The cases (Ev-out), and (Cond) are similar.
\\
- {Cases} (ParB), (StructB) directly follow from the induction hypothesis. 
\\
- No other rules evaluate terms and the proof is trivial.
\end{proof}

\corTheta*
\begin{proof}\ \\
\begin{enumerate}
\item
Immediate; note that for the rule (Node) Lemma~\ref{cor:ThetaB} suffices.
\item
By Theorem~\ref{SRtheorem}, we have that $\nNAFORM{N'}$, so we proceed by
induction on the shape of the derivation of $N \sfreccia N'$ and by cases on the last rule used.
\\
- {Case} (Multi-com) follows directly from the subject reduction Theorem~\ref{SRtheorem}.
%If this rule is applied, than 
%$N$ is in the form 
%\[\!\!\! \nNAFORM{\ell_1 \! : \!  [\OUTM{v_1,\! \cdots \!,v_k}{L}. \, \NIL \  \|\  B_1]\ | \
%             \ell_2  \! : \! [\Sigma^{i}_2 \ \| \ (E_1,\! \cdots \!,E_j;x_{j+1},\! \cdots \!,,x_k).Q \ \| \ B_2]}
%             \] 
%Since 
%$
%\nNAFORM{N}
%$
%we have both 
%$\nPAFORM{\ell_1}{\OUTM{v_1,\! \cdots \!,v_k}{L}. \, \NIL}$ and  the required 
%$\forall \ell' \in L: (\ell_1,  \mess{\hat{v}_1,\cdots,\hat{v}_k}) \in  \kappa(\ell')$, 
%there exists $\hat{G} \in \Theta(\ell)$ such that
%$v_{i\downarrow_2} \in Lang(\hat{v_i})$.
%
%where $\hat{v}_i= v_{i_{\downarrow_2}}$, for all $i$.
\\
- {Cases} (ParN), (StructN), and (Node) directly follow from the induction hypothesis, and for the other rules  the premise is false.
\item
\textcolor{red}{da controllare}
Suppose that $N \xrightarrow{\langle{j,\gamma}\rangle}_{\ell} N'$ then $\gamma \in \alpha_{\ell}(j)$.
By Theorem~\ref{SRtheorem}, we have that $\nNAFORM{N'}$, so we proceed by
induction on the shape of the derivation of $N \sfreccia N'$ and by cases on the last rule used.
\\
- {Case} (A-com)
We have a process with prefix  $\langle{j,\gamma}\rangle$ and therefore $\gamma \in \alpha_{\ell}(j)$, because $\nNAFORM{N}$.
\\
- {Cases} (ParN), (StructN), and (Node) directly follow from the induction hypothesis, and for the other rules  the premise is false.
\end{enumerate}
\end{proof}


%In a completely similar way can be proved the following theorem, whose proof we skip.
%\begin{corollary}\label{cor:kappa}\ \\
%Let $N \xrightarrow{\mess{v_1,\dots,v_n}}_{\ell, \ell'} N'$ denote a reduction in which the message sent by node $\ell$ is received by node $\ell' $.
%\\
%If $\nNFORM{N}$ and \textcolor{blue}{$N \xrightarrow{\mess{v_1,\dots,v_n}}_{\ell,\ell'} N'$ then
%%$(\ell,\mess{\hat{v}_1,\dots,\hat{v}_n}}) \in \kappa(\ell')$, 
%where $\hat{v_i} = 
%\dsem{v_i}^i_{{\Sigma^i_\ell \downarrow_2}}$
%}
%% $\forall \ell' \in L$ 
%%all $E_i$ are evaluated at node $\ell$.
%%If $\nNFORM{N}$ and $N \xrightarrow{E_1, ...,E_n}_\ell  N'$ then $\forall k \in [0,n]$ it is
%%$(\dsem{E_k}^i_{\Sigma^i_\ell})_{\downarrow_2} \, \in \Theta(\ell)$.
%\end{corollary}
%\corKappa*
%\begin{proof}
%By Theorem~\ref{SRtheorem}, we have that $\nNFORM{N'}$, so we proceed by
%induction on the shape of the derivation of $N \rightarrow N'$ and by cases on the last rule used.
%\\
%- {Case} (Multi-com).
%If this rule is applied, than 
%$N$ is in the form 
%\[\!\!\! \nNFORM{\ell_1 \! : \!  [\OUTM{v_1,\! \cdots \!,v_k}{L}. \, \NIL \  \|\  B_1]\ | \
%             \ell_2  \! : \! [\Sigma^{i}_2 \ \| \ (E_1,\! \cdots \!,E_j;x_{j+1},\! \cdots \!,,x_k).Q \ \| \ B_2]}
%             \] 
%Since 
%$
%\nNFORM{N}
%$
%we have both 
%$\nPFORM{\ell_1}{\OUTM{v_1,\! \cdots \!,v_k}{L}. \, \NIL}$ and  the required 
%$\forall \ell' \in L: (\ell,  \mess{\hat{v}_1,\cdots,\hat{v}_k}) \in  \kappa(\ell')$, 
%where $\hat{v}_i= v_{i_{\downarrow_2}}$, for all $i$.
%\\
%- {Cases} (ParN), (StructN), and (Node) directly follow from the induction hypothesis, and for the other rules  the premise is false.
%\hfill$\Box$
%\end{proof}



%\paragraph{Existence of Estimates}


\begin{definition}\label{partialorder}
The set of estimates can be partially ordered by setting \\
$(\hat{\Sigma}_1,\kappa_1, \Theta_1, \alpha_1)$ $\sqsubseteq (\hat{\Sigma}_2,\kappa_2, \Theta_2, \alpha_2)$
iff
\begin{itemize}
\item
$\forall x \in {\mathcal X}_{\ell} \cup {\mathcal I}_{\ell}: \hat{\Sigma}_1(x) \subseteq \hat{\Sigma}_2(x)$

\item
$\forall \ell \in {\mathcal L}: \kappa_1(\ell) \subseteq \kappa_2(\ell)$

\item
$\forall \ell \in {\mathcal L}: \Theta_1(\ell) \subseteq \Theta_2(\ell)$

\item
$\forall j \in {\mathcal J}_\ell, \forall \ell \in {\mathcal L}: \alpha_1(\ell, j) \subseteq \alpha_2(\ell, j)$
\end{itemize}
\end{definition}
This suffices for making the set of proposed
solutions into a complete lattice; 
we write
$(\hat{\Sigma}_1,\kappa_1, \Theta_1, \alpha_1) \sqcup (\hat{\Sigma}_2,\kappa_2, \Theta_2, \alpha_2)$
for the binary least upper bound (defined point-wise),
$\sqcap{\mathcal M}$ for the greatest lower bound of a set ${\mathcal M}$
of proposed solutions (also defined pointwise),
and $(\bot,\bot,\bot,\bot)$ for the least element.

A Moore family ${\mathcal M}$ contains a greatest element ($\sqcap \emptyset$) and a least element ($\sqcap {\mathcal M}$). 
Since the set of analysis estimates constitutes a Moore family, we have that
there always is a least estimate to the specification in \tablename~\ref{analysis}.

%\begin{restatable}[Existence of estimates]{theorem}{extsolutions}\label{Mooretheorem}
%\  \\
%Given $N$ its estimates form a Moore family, hence it has a minimal element.
%\end{restatable}


\extsolutions*
\begin{proof}
Let ${\mathcal M} = \{ (\hat{\Sigma}_r,\kappa_r, \Theta_r, \alpha_r) \}$ a set of estimates for $N$.
We proceed by structural induction on $N$.
\noindent
We have to check that $\sqcap {\mathcal M} = (\hat{\Sigma}',\kappa', \Theta', \alpha') \models N$.
We just consider one case. The others are similar.
\\
- Case $\ell : [B]$.
Since 
$\forall k: (\hat{\Sigma}_r,\kappa_r, \Theta_r, \alpha_r) \models  \ell : [B]$, then 
$(\hat{\Sigma}_r,\kappa_r, \Theta_r, \alpha_r) \models_{_{\ell}}B$.
\noindent
Using the induction hypothesis and the fact that the components of $(\hat{\Sigma}',\kappa', \Theta', \alpha')$ are obtained 
pointwise, it follows that 
$(\hat{\Sigma}',\kappa', \Theta', \alpha') \models_{_{\ell}}B$
thus establishing the required judgement
$(\hat{\Sigma}',\kappa', \Theta', \alpha') \models  \ell : [B]$.
\end{proof}

\trigger*
\begin{proof}
For proving the first item, suppose by contradiction that there exists a transition $N' \rightarrow N''$, derived by using the rule  \mbox{(A-com)}, with action $\gamma$ and actuator $j$. 
Then a control process in $N'$ must include the prefix $\langle{j,\gamma}\rangle$. 
Now, because of Theorem~\ref{SRtheorem}, we have that $\nNAFORM{N}$ implies $\nNAFORM{N'}$. 
As a consequence, the analysis for $N'$ must hold for the process $\OUTS{j,\gamma}{P}$ and therefore $\gamma \in \alpha_{\ell}(j)$: contradiction.

The second item  follows by a similar argument.
\end{proof}

\confine*
\begin{proof}
By contradiction suppose that $N$ is confined and that $N \rightarrow N'$ and that there exists a transition $N' \xrightarrow{\mess{v_1,\dots,v_n}}_{\ell, \ell'} N''$
such that $\exists i : D_{cls}(v_i) = \s$. 
Then, by Corollary~\ref{cor:Theta},
it holds $(\ell,\mess{\hat{v}_1,\dots,\hat{v}_n}) \in \kappa(\ell')$, where $\hat{v}_i = v_{i\downarrow_2}$.
Now, since $N$ is confined, we know that $\forall i. \ S_{cls}(\hat{v}_i) = \p$: contradiction.
\end{proof}


\nrunwd*
\begin{proof}
By contradiction suppose that $N$ safely communicates and that $N \rightarrow N'$ and that there exists a transition $N' \xrightarrow{\mess{v_1,\dots,v_n}}_{\ell, \ell'} N''$
such that $level(\ell) > level(\ell')$. 
Then, by Corollary~\ref{cor:Theta},
it holds $(\ell,\mess{\hat{v}_1,\dots,\hat{v}_n}) \in \kappa(\ell')$, where $\hat{v}_i = v_{i\downarrow_2}$.
Now, since $N$ safely communicates, $level(\ell) \leq level(\ell')$: contradiction.
%
\end{proof}







==> sections/verification.tex <==
% !TEX root = ../main_coord2016.tex

In this section we show how the output of the analysis can be used to verify two classes of system properties.
The first one considers the relationships between the physical and the logical components of a node, in particular how sensors and actuators are used.
Morover, we also check how data are aggegated.
The second subsection shows that some security properties can be verified using our analysis.
In order to deal with cryptography, we extend \IoTLySa\ and its analysis with the needed constructs and definitions.


\subsection{Verifying system activities}
\noindent
\textcolor{red}{
Back again to our example, we have that 
%\[N_{cp} = \ell_{cp} : [ P_{cp} \ \|\ S_{cp}  \ \|\ B_{cp} ] \xrightarrow{1}_{\ell_{cp}} N'_{cp} = \ell_{cp} : [ P'_{cp} \ \|\ S_{cp}  \ \|\ B_{cp} ]\]
%Since $\nNFORM{N_{cp}}$, we have that
$1^{\ell_{cp}} \in \Theta(\ell_{cp})$, where $(\dsem{1}^1_{\Sigma^1_{\ell_{cp}}})_{\downarrow_2} = 1^{\ell_{cp}}$,  
%$P'_{cp} = (z' := noiseRed(v)).\OUTM{z'}{\{\ell_a\}}.P''_{cp}$, 
and where $v$ is the actual value received by the first sensor.
Similarly, we have that
%\[
%\begin{array}{c}
%\ell_{cp} : [ \OUTM{z'}{\{\ell_a\}}.P''_{cp} \ \|\ S_{cp}  \ \|\ B_{cp} ] \mid 
%\ell_a : [\ \mu h. \INPS{}{x}{\OUTM{car, x}{\{\ell_s\}.\ h}} \ \|\ B_{a}\ ]
%\\
%\xrightarrow{v}_{\ell_{cp},\ell_a} \\
%\ell_{cp} : [ P''_{cp} \ \|\ S_{cp}  \ \|\ B_{cp} ] \mid 
%\ell_a : [\OUTM{car, v}\{\ell_s\}.P'_{a} \ \|\ B_{a}\ ]
%\end{array}
%\]
%Since $\nNFORM{N_{cp} \mid N_a}$, we have that 
$(\ell_{cp},\mess{\hat{v}}) \in \kappa(\ell_{a})$, 
where $\hat{v} = v_{\downarrow_2}$.
}


Our first property concerns the usage of sensors and permits a designer to either detect a sensor to be superfluous or to discover a flaw in the code.

\begin{definition}
Let $N$ be the node $\ell:[B]$ containing the sensor $i$. \\
The node $N$ {\em never uses} the sensor $i$ if and only if whenever
$N \rightarrow^* N'$ then there is no transition
$N' \xrightarrow{E_1, ...,E_r}_\ell N''$ in which $i$ occurs in $E_k$ for some $k \in [1,r]$.
\end{definition}


%\begin{restatable}[]{thm}{trigger}\label{Triggertheorem}
%Let $N$ be the node $\ell:[B]$ containing the actuator $j$, and let $\nNAFORM{N}$. 
%\begin{enumerate}
%\item
%If $\gamma \not\in \alpha_{\ell}(j)$, then 
%$N$  never fires the action $\gamma$ of $j$.
%\item
%If $\alpha_{\ell}(j) = \emptyset$, then the actuator $j$ is never used.
%\end{enumerate}
%\end{restatable}


We now show how the component  $\alpha$ allows us to perform other checks on actuators that 
might suggest to use a simpler actuator if some of its actions are never triggered, or even to remove it if it is never used.
In the following definitions  $\rightarrow^*$ denotes
the reflexive and transitive closure of $\rightarrow$.

\begin{definition}
Let $N$ be the node $\ell:[B]$ containing the actuator $j$.
\begin{itemize}
\item
The node $N$ {\em never fires} the action $\gamma$ of $j$ if and only if whenever
$N \rightarrow^* N'$ then there is no transition
$N' \xrightarrow{\langle{j,\gamma}\rangle}_{\ell} N''$.
\item
The actuator $j$ is \emph{never used} if and only if for all actions $\gamma$ of $j$, $N$ never fires $\gamma$.
\end{itemize}
\end{definition}

%
%
Since we are over-approximating, the presence of $\gamma$ in $\alpha_{\ell}(j)$ only implies that the node {\em may} trigger the action $\gamma$ on actuator $j$.
\textcolor{red}{
In our running example, the inclusion
$\{\mathsf{turnon},\mathsf{turnoff}\} \subseteq \alpha_{_{\ell_{p}}}(5)$ only says that the two actions are reachable.
Instead if, e.g.~the output $\mess{5,\mathsf{turnoff}}$ were erroneously omitted in the last line of the specification of process $P_{p,1}$, then our CFA
would detect that $\mathsf{turnoff} \not\in \alpha_{_{\ell_{p}}}(5)$.
}

\begin{restatable}[]{thm}{trigger}\label{Triggertheorem}
Let $N$ be the node $\ell:[B]$ containing the actuator $j$, and let $\nNAFORM{N}$. 
\begin{enumerate}
\item
If $\gamma \not\in \alpha_{\ell}(j)$, then 
$N$  never fires the action $\gamma$ of $j$.
\item
If $\alpha_{\ell}(j) = \emptyset$, then the actuator $j$ is never used.
\end{enumerate}
\end{restatable}
%
\alert{
Credo che ci vogliano 2 palle sulla generazione dei constraints e sulla loro soluzione, ma non ci ho pensato affatto.
Come si fa? Vedi il formato dei Nielson: Layered Fixed Point Logic, 2010 + Corr
}





